Approximately multiplicative maps from weighted semilattice algebras

We investigate which weighted convolution algebras $\ell^1_\omega(S)$, where $S$ is a semilattice, are AMNM in the sense of Johnson (JLMS, 1986). We give an explicit example where this is not the case. We show that the unweighted examples are all AMNM, as are all $\ell^1_\omega(S)$ where $S$ has either finite width or finite height. Some of these finite-width examples are isomorphic to function algebras studied by Feinstein (IJMMS, 1999). We also investigate when $(\ell^1_\omega(S),{\bf M}_2)$ is an AMNM pair in the sense of Johnson (JLMS, 1988), where ${\bf M}_2$ denotes the algebra of 2-by-2 complex matrices. In particular, we obtain the following two contrasting results: (i) for many non-trivial weights on the totally ordered semilattice ${\bf N}_{\min}$, the pair $(\ell^1_\omega({\bf N}_{\min}),{\bf M}_2)$ is not AMNM; (ii) for any semilattice $S$, the pair $(\ell^1(S),{\bf M}_2)$ is AMNM. The latter result requires a detailed analysis of approximately commuting, approximately idempotent $2\times 2$ matrices.

==> WSamnm_forme.tex <==

% shameless hack to force page break in personal version
\newcommand{\newpageinarx}{\vfill\eject}


\usepackage{mathpazo}
%\usepackage{concrete}

%-------------
\RequirePackage{amsthm}   %Inbuilt environments for defns etc
%\usepackage{theorem}

\newcounter{pulse}[section]
\numberwithin{pulse}{section}  % all thms, etc set from pulse
%Styles for theorems, definitions, remarks
\newcommand{\thf}{\bf} % alias for theorem heading font
%-Theorems
\theoremstyle{plain}
\newtheorem{thm}[pulse]{\thf Theorem}
\newtheorem{prop}[pulse]{\thf Proposition}
\newtheorem{lem}[pulse]{\thf Lemma}
\newtheorem{cor}[pulse]{\thf Corollary}
%-Definitions
\theoremstyle{definition}
\newtheorem{dfn}[pulse]{\thf Definition}
\newtheorem*{notn}{\thf Notation}
\newtheorem{eg}[pulse]{\thf Example}
%-Remarks
\theoremstyle{remark}
\newtheorem{rem}[pulse]{\thf Remark}
\newtheorem*{remstar}{\thf Remark}

%--------------------------


%\usepackage[notref,notcite]{showkeys}
%\usepackage{fancyhdr}
%\pagestyle{fancy}
%\lhead{}
%\rhead{\sc Final version before 1st submission (with some private comments)}

%% - margin hacks by hand
\setlength{\textwidth}{\paperwidth}
\addtolength{\textwidth}{-60mm}
\setlength{\oddsidemargin}{5mm}
\setlength{\evensidemargin}{5mm}
\setlength{\topmargin}{-8mm}

\setlength{\textheight}{\paperheight}
\addtolength{\textheight}{-60mm}
\setlength{\footskip}{15mm}


%% FOUND AT
%% http://mintaka.sdsu.edu/GF/bibliog/latex/floats.html
%
% Alter some LaTeX defaults for better treatment of figures:
    % See p.105 of "TeX Unbound" for suggested values.
    % See pp. 199-200 of Lamport's "LaTeX" book for details.
    %   General parameters, for ALL pages:
    \renewcommand{\topfraction}{0.9}	% max fraction of floats at top
    \renewcommand{\bottomfraction}{0.8}	% max fraction of floats at bottom
    %   Parameters for TEXT pages (not float pages):
    \setcounter{topnumber}{2}
    \setcounter{bottomnumber}{2}
    \setcounter{totalnumber}{4}     % 2 may work better
    \setcounter{dbltopnumber}{2}    % for 2-column pages
    \renewcommand{\dbltopfraction}{0.9}	% fit big float above 2-col. text
    \renewcommand{\textfraction}{0.07}	% allow minimal text w. figs
    %   Parameters for FLOAT pages (not text pages):
    \renewcommand{\floatpagefraction}{0.7}	% require fuller float pages
	% N.B.: floatpagefraction MUST be less than topfraction !!
    \renewcommand{\dblfloatpagefraction}{0.7}	% require fuller float pages

	% remember to use [htp] or [htpb] for placement





\usepackage{sectsty}
\allsectionsfont{\sc}
\numberwithin{equation}{section}

\usepackage[usenames]{color}
\renewcommand{\dt}[1]{\textcolor{Bittersweet}{\sf#1}}

% hack to get round \paragraph being unsupported in other class files
\newcommand{\para}[1]{\paragraph{#1}}

%\newcommand{\YCrem}[1]{\textcolor{Blue}{\sf#1}}
\newcommand{\YCrem}[1]{}

% doing a Hasse diagram to sort out logic of Section 5
% load up Paul Taylor's diagram.sty macros
\RequirePackage[PS,nohug]{diagrams}
% this should now avoid annoying label rotation

%\openup3pt


==> WSamnm_mainmac2.tex <==
% from YCmath.sty
\NeedsTeXFormat{LaTeX2e}
\RequirePackage{amsmath,amssymb,amsfonts}
\renewcommand{\emph}[1]{{\sl #1}\/} % use slanted font for emphasis

\newcommand{\st}{\;:\;}
\newcommand{\defeq}{:=}
\newcommand{\dt}[1]{{\sf {#1}}}

% journals seem to want upright roman numerals in numbered lists, we need to force this if in an italic environment
\newenvironment{YCnum}{%
\begin{enumerate}
\renewcommand{\labelenumi}{{\rm(\roman{enumi})}}
\renewcommand{\theenumi}{{\rm(\roman{enumi})}}
}{\end{enumerate}\ignorespacesafterend}


%%Personal preference and fundamentals
\newcommand{\veps}{\varepsilon}
\newcommand{\wtild}{\widetilde}
\newcommand{\what}{\widehat}
\newcommand{\blob}{\bullet}
\newcommand{\blank}{\underline{\quad}}

\newcommand{\tr}{\operatorname{Tr}} % matrix trace
\newcommand{\iso}{\cong}
%\renewcommand{\Re}{\operatorname{\sf Re}}
%\renewcommand{\Im}{\operatorname{\sf Im}}
\newcommand{\tp}{\mathop{\otimes}\nolimits}
\newcommand{\id}[1][]{{\sf 1}_{#1}} % identity of group, algebra, object in category
\newcommand{\wstar}{\ensuremath{{\rm w}^*}}

\newcommand{\ptp}{\mathop{\widehat{\otimes}}\nolimits} % projective tensor product

\newcommand{\abs}[1]{\vert{#1}\vert}
\newcommand{\Abs}[1]{\left\vert{#1}\right\vert}
\newcommand{\norm}[1]{\Vert{#1}\Vert}
\newcommand{\Norm}[1]{\left\Vert{#1}\right\Vert}

\newcommand{\Bdd}{{\mathcal B}}

\newcommand{\Cplx}{\mathbb C}
\newcommand{\Nat}{\mathbb N}
\newcommand{\Zahl}{\mathbb Z}
\newcommand{\Disc}{\mathbb D} %Open unit disc
\newcommand{\Torus}{\mathbb T} %Unit circle

\newcommand{\Cst}{\operatorname{C}^*}
%----------------------------

\newcommand{\Lin}{{\mathcal L}}

\newcommand{\TFAE}{The following are equivalent}
\newcommand{\WLOG}{without loss of generality}


\newcommand{\Nmax}{{\mathbb N}_{\vee}}
\newcommand{\lm}{\lambda}


\newcommand{\Mult}{\operatorname{Mult}}

\newcommand{\diff}{{\operatorname{def}}} % multiplicative defect
\newcommand{\al}{\alpha}
\newcommand{\om}{\omega}
\newcommand{\gm}{\gamma}
\newcommand{\kp}{\kappa}
\newcommand{\Lm}{\Lambda}
\newcommand{\Ind}{{\mathbb I}}

\newcommand{\Nmin}{{\mathbb N}_{\min}}
\newcommand{\clB}{\overline{\mathbb B}^{\rm HS}}
\newcommand{\clD}{\overline{\mathbb D}}
\newcommand{\oD}{{\mathbb D}}

\newcommand{\gen}[2][]{\langle#2\rangle_{#1}}
\newcommand{\FG}[1]{({\rm FG}_{#1})}
\newcommand{\Sfix}{S_{\rm fix}}
\newcommand{\free}[1]{{\bf 2}^{[#1]}_*}  % free semilattice on #1 generators

\newcommand{\twomat}[4]{\left(\begin{matrix} #1 & #2 \\ #3 & #4 \end{matrix}\right)}
\newcommand{\Mat}[1]{{\mathbb M}_{#1}}
\newcommand{\sT}{{\bf T}}

\newcommand{\dist}{\operatorname{dist}}
\newcommand{\lom}{\ell^1_\om}

%\newcommand{\vrb}{\operatorname{vb}}
%\newcommand{\prol}{\operatorname{prol}}

\newcommand{\hm}{homo\-morphism}
\newcommand{\hsnorm}[1]{\norm{#1}_{\rm HS}}
\newcommand{\hsNorm}[1]{\Norm{#1}_{\rm HS}}
\newcommand{\opnorm}[1]{\norm{#1}_{\rm op}}

%\newcommand{\base}[1]{\theta(#1)} % original notation
\newcommand{\base}[1]{\widetilde{#1}} % newer notation

\newcommand{\te}{\base{e}}
\newcommand{\tf}{\base{f}}
\newcommand{\tg}{\base{g}}
\newcommand{\thp}{\base{p}}
\newcommand{\tq}{\base{q}}
\newcommand{\tx}{\base{x}}
\newcommand{\ty}{\base{y}}
\newcommand{\tef}{\base{ef}}
\newcommand{\tfe}{\base{fe}}
\newcommand{\tfg}{\base{fg}}
\newcommand{\tgf}{\theta(gf)}
\newcommand{\tefe}{\theta(efe)}
\newcommand{\tefg}{\theta(efg)}




